Spin-polarizing electron beam splitter from crossed graphene nanoribbons

Junctions composed of two crossed graphene nanoribbons (GNRs) have been theoretically proposed as electron beam splitters where incoming electron waves in one GNR can be split coherently into propagating waves in \emph{two} outgoing terminals with nearly equal amplitude and zero back-scattering. Here we scrutinize this effect for devices composed of narrow zigzag GNRs taking explicitly into account the role of Coulomb repulsion that leads to spin-polarized edge states within mean-field theory. We show that the beam-splitting effect survives the opening of the well-known correlation gap and, more strikingly, that a \emph{spin-dependent} scattering potential emerges which spin-polarizes the transmitted electrons in the two outputs. A near-perfect polarization can be achieved by joining several junctions in series. Our findings suggest that GNRs are interesting building blocks in spintronics and quantum technologies with applications for interferometry and entanglement.

==> latexmkrc <==
$ENV{'TEXINPUTS'}='./tex//:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./bst//:' . $ENV{'BSTINPUTS'};

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
